GPTVoiceTasker: Advancing Multi-step Mobile Task Efficiency Through Dynamic Interface Exploration and Learning

Virtual assistants have the potential to play an important role in helping users achieves different tasks. However, these systems face challenges in their real-world usability, characterized by inefficiency and struggles in grasping user intentions. Leveraging recent advances in Large Language Models (LLMs), we introduce GptVoiceTasker, a virtual assistant poised to enhance user experiences and task efficiency on mobile devices. GptVoiceTasker excels at intelligently deciphering user commands and executing relevant device interactions to streamline task completion. The system continually learns from historical user commands to automate subsequent usages, further enhancing execution efficiency. Our experiments affirm GptVoiceTasker's exceptional command interpretation abilities and the precision of its task automation module. In our user study, GptVoiceTasker boosted task efficiency in real-world scenarios by 34.85%, accompanied by positive participant feedback. We made GptVoiceTasker open-source, inviting further research into LLMs utilization for diverse tasks through prompt engineering and leveraging user usage data to improve efficiency.

==> Evaluation.tex <==
\begin{table}[]
\begin{tabular}{cccc}
\hline
\textbf{Hit rate@k} & \textbf{No of Success} & \textbf{No of Fail} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Percentage\\  of Success\end{tabular}}} \\ \hline
\textit{k = 1} & 38 & 12 & 76\% \\ 
\textit{k = 3} & 41 & 9 & 82\% \\ \hline
\end{tabular}
\caption{The experiment results with k = 1 and k = 3 for 50 test cases.}
\label{table:result}
\end{table}

==> Usecases.tex <==
\section{A Use Case Scenario}
\label{sec:usecases}

In this section, we use the example in Fig.~\ref{fig:thumbnail_image} to demonstrate how \tool is useful in real-world scenario. The example includes usages of both direct feature invocation and background virtual assistant to completely replace physical interactions, which also applies to many other circumstances.

Cindy, as a mom of two kids, always has her hands busy with multiple tasks from cooking to cleaning all day long. As Cindy is passionate about cooking for her children, she often reaches out to her phone when preparing the meal to check for cooking ingredients and instructions. However, it is quite inconvenient for her to pick up the phone as her hands are often occupied when holding kitchen accessories. In addition, uncleanliness is a major concern to her hence she has to wash and dry her hands before and after touching the phone screen. Sometimes, her cooking glove prevents her from tapping on the screen or causing her to make imprecise tap. The whole cooking process is exhausted and unproductive, and she faced the same issue every day.

Cindy is introduced to \tool, and quickly learned how to use the tool effectively. When cooking, Cindy can entirely use her voice to navigate between different apps in the smartphone. With other virtual assistant such as Voice Access, Cindy would have to navigate through many screens with multiple interaction to view her saved recipes. Using \tool, she can directly view all her saved recipes in the World Cuisines app with a single voice command, hence saving a lot of time and efforts. For choosing the Healthy Burger recipe, she can provide short-form command "Press Healthy Burger", \tool will virtually tap on desire UI element and provide her with audio feedback. 

